Joint Modeling of Code-Switched and Monolingual ASR via Conditional Factorization

Conversational bilingual speech encompasses three types of utterances: two purely monolingual types and one intra-sententially code-switched type. In this work, we propose a general framework to jointly model the likelihoods of the monolingual and code-switch sub-tasks that comprise bilingual speech recognition. By defining the monolingual sub-tasks with label-to-frame synchronization, our joint modeling framework can be conditionally factorized such that the final bilingual output, which may or may not be code-switched, is obtained given only monolingual information. We show that this conditionally factorized joint framework can be modeled by an end-to-end differentiable neural network. We demonstrate the efficacy of our proposed model on bilingual Mandarin-English speech recognition across both monolingual and code-switched corpora.

==> figures/subnet.tex <==
% \begin{filecontents}{data.csv}
% A,  B,  C,  D
% 1,  10, 1,  1
% 10, 9,  1,  1
% 0,  ,  1,  0
% 0,  0,  0,  1
% \end{filecontents}
% \pgfplotstableread[col sep=comma,]{data.csv}\datatable

% % \begin{document}
% \resizebox {\linewidth} {!} {
% \begin{tikzpicture}
% \begin{axis}[width=11cm,
%     ybar,
%     bar width=7pt,
%     xlabel={A},
%     % xtick=data,
%     % xticklabels from table={\datatable}{A},
%     xtick=data,
%     xticklabels={Cond RNN-T, Cond RNN-T + LS, Mono Zh CTC, Mono En CTC},
%     ymajorgrids,
%     legend pos=north east
%              ]
%     \addplot table [x expr=\coordindex, y=A]{\datatable};
%     \addplot table [x expr=\coordindex, y=B]{\datatable};
%     \addplot table [x expr=\coordindex, y=C]{\datatable};
%     \addplot table [x expr=\coordindex, y=D]{\datatable};
%     \legend{Cond RNN-T, Cond RNN-T + LS, Mono Zh CTC, Mono En CTC}
% \end{axis}
% \end{tikzpicture}
% }

\resizebox {\linewidth} {!} {
% \begin{figure}[ht!]
    % \centering
    % \subfloat[][Sub figure first]{\resizebox{0.5\textwidth}{!}{
\begin{tikzpicture}
    \begin{axis}[
        ybar,
        ymin=0,
        width  = 5cm,
        height = 5cm,
        bar width=5pt,
        ylabel={CER},
        nodes near coords,
        % xticklabel style={rotate=90},
        xtick = data,
        table/header=false,
        table/row sep=\\,
        xticklabels from table={\footnotesize
          wells\\\footnotesize lemput\\\footnotesize wang\\
          }{[index]0},
        enlarge y limits={value=0.2,upper}
      %  legend pos=north west
    ]
    %  \legend{1\%, 5\%}
    \addplot table[x expr=\coordindex,y index=0]{3.9\\4.1\\100\\};
    % \addplot table[x expr=\coordindex,y index=0]{3\\2\\8\\};
    % \pgfplotsinvokeforeach{0,3,4,7,8,11}{\coordinate(l#1)at(axis cs:#1,0);}
    \end{axis}
    \coordinate(bbs)at(current bounding box.south);
    % \foreach[count=\i,evaluate={\s=int(4*\i-1)},evaluate={\e=int(4*(\i-1))}] \text in {Axial,Coronial,Sagittarial}
    %   \draw[decorate,decoration=brace]([xshift=8pt]l\s|-bbs)--node[below=5pt]{\text}([xshift=-8pt]l\e|-bbs);
\end{tikzpicture}
    % A blank line here like a new paragraph so next picture is placed below
    % \subfloat[][Sub figure second]{\resizebox{0.5\textwidth}{!}{

\begin{tikzpicture}
    \begin{axis}[
        ybar,
        ymin=0,
        width  = 5cm,
        height = 5cm,
        bar width=5pt,
        ylabel={WER},
        nodes near coords,
        % xticklabel style={rotate=90},
        xtick = data,
        table/header=false,
        table/row sep=\\,
        xticklabels from table={\footnotesize
          wells\\\footnotesize lemput\\\footnotesize wang\\
          }{[index]0},
        enlarge y limits={value=0.2,upper}
      %  legend pos=north west
    ]
    %  \legend{1\%, 5\%}
    \addplot table[x expr=\coordindex,y index=0]{3.9\\4.1\\100\\};
    % \addplot table[x expr=\coordindex,y index=0]{3\\2\\8\\};
    % \pgfplotsinvokeforeach{0,3,4,7,8,11}{\coordinate(l#1)at(axis cs:#1,0);}
    \end{axis}
    % \coordinate(bbs)at(current bounding box.south);
    % \foreach[count=\i,evaluate={\s=int(4*\i-1)},evaluate={\e=int(4*(\i-1))}] \text in {Axial,Coronial,Sagittarial}
    %   \draw[decorate,decoration=brace]([xshift=8pt]l\s|-bbs)--node[below=5pt]{\text}([xshift=-8pt]l\e|-bbs);
\end{tikzpicture}
    % A blank line here like a new paragraph so next picture is placed below
    % \subfloat[][Sub figure second]{\resizebox{0.5\textwidth}{!}{
}

==> scratch.tex <==
% Rather than treating code-switched ASR as a single sequence transduction task, we formulate it using three portions: 1) recognizing Mandarin 2) recognizing English and 3) composing recognized monolingual segments into a code-switched sequence. Our method jointly estimates the probability $P(\mathbf{y}, \mathbf{y}^M, \mathbf{y}^E|\mathbf{x})$ of the code-switched sequence, $\mathbf{y}$, and the monolingual sequences that it consists of, $\mathbf{y}^M$ and $\mathbf{y}^E$ where $y_l^M \in \mathcal{V}^M$ and $y_l^E \in \mathcal{V}^E$. This factorizes into the monolingual probabilities, $P(\mathbf{y}^M|\mathbf{x})$ and $P(\mathbf{y}^E|\mathbf{x})$, and the code-switched probability $P(\mathbf{y}|\mathbf{y}^M, \mathbf{y}^E)$ as follows:

% \begin{align}
%     % P(\mathbf{y}, \mathbf{y}^M, \mathbf{y}^E|\mathbf{x}) &= P(\mathbf{y}|\mathbf{y}^M, \mathbf{y}^E)P(\mathbf{y}^M|\mathbf{x})P(\mathbf{y}^E|\mathbf{x}) \\
%     P(\mathbf{y}, \mathbf{y}^M, \mathbf{y}^E|\mathbf{x}) &= P(\mathbf{y}|\mathbf{y}^M, \mathbf{y}^E, \mathbf{x})P(\mathbf{y}^M|\mathbf{x})P(\mathbf{y}^E|\mathbf{x})
%     % P(\mathbf{y}^M|\mathbf{x}) &= \sum_{\mathbf{z}^M \in \mathcal{Z}^M} P(\mathbf{z}^M | \mathbf{x}) \\
%     % P(\mathbf{y}^E|\mathbf{x}) &= \sum_{\mathbf{z}^E \in \mathcal{Z}^E} P(\mathbf{z}^E | \mathbf{x}) \\
%     % P(\mathbf{y}|\mathbf{y}^M, \mathbf{y}^E, \mathbf{x}) &= \sum_{\mathbf{z}, \mathbf{z}^M, \mathbf{z}^E \in \mathcal{Z}'} P(\mathbf{z} |\mathbf{z}^M, \mathbf{z}^E)P(\mathbf{z}^M|\mathbf{x})P(\mathbf{z}^E|\mathbf{x})
%     % P(\mathbf{y}^M|\mathbf{x}) &= \sum_{\mathbf{z}^M \in \mathcal{Z}^M} \prod_{i=1}^{T} P(z_i^M | \mathbf{x}) \\
%     % P(\mathbf{y}^E|\mathbf{x}) &= \sum_{\mathbf{z}^E \in \mathcal{Z}^E} \prod_{i=1}^{T} P(z_i^E | \mathbf{x}) \\
%     % P(\mathbf{y}|\mathbf{y}^M, \mathbf{y}^E, \mathbf{x}) &= \sum_{\mathbf{z} \in \mathcal{Z}} \prod_{i=1}^{T+L} P(z_i | \mathbf{z}^M, \mathbf{z}^E, y_{1:i-1})
% \end{align}

% Scratch:
% \begin{align}
%     P(\mathbf{y, \mathbf{y}^M, \mathbf{y}^E}|\mathbf{x}) &= \sum_{\mathbf{z}' \in \mathcal{Z}'} P(\mathbf{z}, \mathbf{z}^M, \mathbf{z}^E | \mathbf{x}) \\
%     P(\mathbf{z}, \mathbf{z}^M, \mathbf{z}^E|\mathbf{x}) &= P(\mathbf{z} |\mathbf{z}^M, \mathbf{z}^E)P(\mathbf{z}^M|\mathbf{x})P(\mathbf{z}^E|\mathbf{x})
% \end{align}

% \begin{align}
%     P(\mathbf{z}^M|\mathbf{x}) &= P(\mathbf{z}^M|\mathbf{h}^M) P(\mathbf{h}^M|\mathbf{x}) \\
%     P(\mathbf{z}^E|\mathbf{x}) &= P(\mathbf{z}^E|\mathbf{h}^E) P(\mathbf{h}^E|\mathbf{x}) \\
%     P(\mathbf{z}, \mathbf{z}^M, \mathbf{z}^E|\mathbf{x}) &= P(\mathbf{z} |\mathbf{h}^M, \mathbf{h}^E) P(\mathbf{h}^M|\mathbf{x}) P(\mathbf{h}^E|\mathbf{x}) \\
%     % P(\mathbf{z}|\mathbf{h}^M, \mathbf{h}^E) &= \prod_{i=1}^{T+L} P(z_i | \mathbf{h}^M, \mathbf{h}^E, \cancel{\mathbf{x}}, z_{1:i-1})
% \end{align}

% \begin{align}
%     \mathcal{L}_{M} &= \textsc{CTCLoss}(\mathbf{z}^M, \mathbf{y}^M) \\
%     \mathcal{L}_{E} &= \textsc{CTCLoss}(\mathbf{z}^E, \mathbf{y}^E) \\
%     \mathcal{L}_{CS} &= \textsc{RNNTLoss}(\mathbf{z}, \mathbf{y}) \\
%     \mathcal{L} &= \mathcal{L}_{CS} + \alpha\mathcal{L}_{M} + \alpha\mathcal{L}_{E}
% \end{align}

% \begin{align}
%     P(\mathbf{z}|\mathbf{x}) = P(\mathbf{z}, \mathbf{z}^M, \mathbf{z}^E|\mathbf{x}) &= P(\mathbf{z}|\mathbf{z}^M, \mathbf{z}^E, \mathbf{x}) P(\mathbf{z}^E, \mathbf{z}^M | \mathbf{x}) \\
%     P(\mathbf{z}|\mathbf{x}) &= P(\mathbf{z} |\mathbf{z}^M, \mathbf{z}^E)P(\mathbf{z}^M|\mathbf{x})P(\mathbf{z}^E|\mathbf{x}) \\
%     P(\mathbf{z}^M|\mathbf{x}) &= P(\mathbf{z}^M|\mathbf{h}^M) P(\mathbf{h}^M|\mathbf{x}) \\
%     P(\mathbf{z}^E|\mathbf{x}) &= P(\mathbf{z}^E|\mathbf{h}^E) P(\mathbf{h}^E|\mathbf{x})
% \end{align}

% \begin{align}
%     P(\mathbf{z}|\mathbf{x}) = P(\mathbf{z}, \mathbf{z}^M, \mathbf{z}^E|\mathbf{x}) &= P(\mathbf{z}|\mathbf{z}^M, \mathbf{z}^E, \mathbf{x}) P(\mathbf{z}^E, \mathbf{z}^M | \mathbf{x}) \\
%     P(\mathbf{z}|\mathbf{x}) &= P(\mathbf{z} |\mathbf{h}^M, \mathbf{h}^E)P(\mathbf{h}^M|\mathbf{x})P(\mathbf{h}^E|\mathbf{x})
% \end{align}

% Note that although the final code-switched sequence probability is computed auto-regressively, we apply the conditional independence assumption to the monolingual sequences. 
% This allows us to maximize the likelihood of the monolingual sequences using the CTC loss \cite{graves2006connectionist} while still using the RNN-T loss \cite{rnnt_graves} to maximize the likelihood of the final code-switched sequence using a multi-tasking scheme.


